SODiff: Semantic-Oriented Diffusion Model for JPEG Compression Artifacts Removal

JPEG, as a widely used image compression standard, often introduces severe visual artifacts when achieving high compression ratios. Although existing deep learning-based restoration methods have made considerable progress, they often struggle to recover complex texture details, resulting in over-smoothed outputs. To overcome these limitations, we propose SODiff, a novel and efficient semantic-oriented one-step diffusion model for JPEG artifacts removal. Our core idea is that effective restoration hinges on providing semantic-oriented guidance to the pre-trained diffusion model, thereby fully leveraging its powerful generative prior. To this end, SODiff incorporates a semantic-aligned image prompt extractor (SAIPE). SAIPE extracts rich features from low-quality (LQ) images and projects them into an embedding space semantically aligned with that of the text encoder. Simultaneously, it preserves crucial information for faithful reconstruction. Furthermore, we propose a quality factor-aware time predictor that implicitly learns the compression quality factor (QF) of the LQ image and adaptively selects the optimal denoising start timestep for the diffusion process. Extensive experimental results show that our SODiff outperforms recent leading methods in both visual quality and quantitative metrics. Code is available at: https://github.com/frakenation/SODiff

==> figs/live1_church/figure_code.tex <==
% 在文档导言区添加必要的包
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{array}

% 图片排版代码
\begin{figure*}[t]
    \centering
    
    \begin{tabular}{c@{\hspace{0.5cm}}c}
        % 左列：LQ图片（带红框）
        \begin{minipage}{0.35\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figs/texture/live1_church/LQ.png}
            \captionof{subfigure}{LQ}
            \label{subfig:lq}
        \end{minipage}
        &
        % 右列：方法结果图片（2行4列)
        \begin{minipage}{0.6\textwidth}
            \centering
            
            % 图片网格
            \begin{tabular}{@{cccc}@{}}
                \includegraphics[width=0.22\textwidth]{figs/texture/live1_church/LQ_with_box.png} & \includegraphics[width=0.22\textwidth]{figs/texture/live1_church/diffbir.png} & \includegraphics[width=0.22\textwidth]{figs/texture/live1_church/fbcnn.png} & \includegraphics[width=0.22\textwidth]{figs/texture/live1_church/hq.png} \\
                \scriptsize LQ_with_box & \scriptsize diffbir & \scriptsize fbcnn & \scriptsize hq \\
                [0.3cm]
                \includegraphics[width=0.22\textwidth]{figs/texture/live1_church/jdec.png} & \includegraphics[width=0.22\textwidth]{figs/texture/live1_church/promptcir.png} & \includegraphics[width=0.22\textwidth]{figs/texture/live1_church/sodiff.png} & \includegraphics[width=0.22\textwidth]{figs/texture/live1_church/supir.png} \\
                \scriptsize jdec & \scriptsize promptcir & \scriptsize sodiff & \scriptsize supir \\
            \end{tabular}
        \end{minipage}
    \end{tabular}
    
    \caption{不同超分辨率方法的视觉比较。左图显示了低质量输入图像，红框标注了用于比较的区域。右侧显示了该区域在不同方法下的超分辨率结果。}
    \label{fig:comparison}
\end{figure*}

==> figs/urban_051/figure_code.tex <==
% 在文档导言区添加必要的包
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{array}

% 图片排版代码
\begin{figure*}[t]
    \centering
    
    \begin{tabular}{c@{\hspace{0.5cm}}c}
        % 左列：LQ图片（带红框）
        \begin{minipage}{0.35\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figs/texture/urban_051/LQ.png}
            \captionof{subfigure}{LQ}
            \label{subfig:lq}
        \end{minipage}
        &
        % 右列：方法结果图片（2行4列)
        \begin{minipage}{0.6\textwidth}
            \centering
            
            % 图片网格
            \begin{tabular}{@{cccc}@{}}
                \includegraphics[width=0.22\textwidth]{figs/texture/urban_051/LQ_with_box.png} & \includegraphics[width=0.22\textwidth]{figs/texture/urban_051/SODiff.png} & \includegraphics[width=0.22\textwidth]{figs/texture/urban_051/diffbir.png} & \includegraphics[width=0.22\textwidth]{figs/texture/urban_051/fbcnn.png} \\
                \scriptsize LQ_with_box & \scriptsize SODiff & \scriptsize diffbir & \scriptsize fbcnn \\
                [0.3cm]
                \includegraphics[width=0.22\textwidth]{figs/texture/urban_051/hq.png} & \includegraphics[width=0.22\textwidth]{figs/texture/urban_051/jdec.png} & \includegraphics[width=0.22\textwidth]{figs/texture/urban_051/lq1.png} & \includegraphics[width=0.22\textwidth]{figs/texture/urban_051/promptcir.png} \\
                \scriptsize hq & \scriptsize jdec & \scriptsize lq1 & \scriptsize promptcir \\
            \end{tabular}
        \end{minipage}
    \end{tabular}
    
    \caption{不同超分辨率方法的视觉比较。左图显示了低质量输入图像，红框标注了用于比较的区域。右侧显示了该区域在不同方法下的超分辨率结果。}
    \label{fig:comparison}
\end{figure*}
